Entities as Experts: Sparse Memory Access with Entity Supervision

We focus on the problem of capturing declarative knowledge about entities in the learned parameters of a language model. We introduce a new model - Entities as Experts (EAE) - that can access distinct memories of the entities mentioned in a piece of text. Unlike previous efforts to integrate entity knowledge into sequence models, EAE's entity representations are learned directly from text. We show that EAE's learned representations capture sufficient knowledge to answer TriviaQA questions such as "Which Dr. Who villain has been played by Roger Delgado, Anthony Ainley, Eric Roberts?", outperforming an encoder-generator Transformer model with 10x the parameters. According to the LAMA knowledge probes, EAE contains more factual knowledge than a similarly sized BERT, as well as previous approaches that integrate external sources of entity knowledge. Because EAE associates parameters with specific entities, it only needs to access a fraction of its parameters at inference time, and we show that the correct identification and representation of entities is essential to EAE's performance.

==> background_original.tex <==
\section{Background}\label{sec:background}



\paragraph{Entity-augmented language models}

Our work is most closely related to \cite{Peters2019-pe} that introduce \knowbert a Bert based \cite{bert} masked language model with a ``Knowledge Attention and Recontextualization'' (KAR) layer that is similar to our entity memory layer. The main difference is in the training setup: \knowbert initializes their model with BERT and use pre-trained entity embeddings to initialize their entity embeddings. They then use a complex training setup which involves several steps of freezing and unfreezing of different components of the model. In contrast, all the parameters in our model are trained from scratch and we do not freeze them, including at fine-tuning time. In addition, \knowbert relies on an external, fixed mention selector whereas we learn a mention boundary predictor.
Earlier attempts to integrate knowledge base information in language models \cite{ahn2016neural, yang2016reference, logan2019barack} are less directly related to our approach.

\paragraph{Memory augmented neural networks}

Our entity memory layers is closely tied to memory-based neural layers \cite{memory_networks, e2e_memory_networks}. In particular, it can be seen as a memory network where memory access is supervised through entity linking, and memory slots each correspond to a learned entity representation. \cite{largepkm} improve the scalability of memory networks by introducing product-key memories, which uses product-keys to efficiently index a large store of values. %

\paragraph{Conditional computation}

\tf{TOo similar to PKM?}
Conditional computation models seek to increase model capacity without a proportional increase in computational complexity. This is usually done through routing, where for only a subset of the network is used to process each input. To facilitate such routing, different approaches have been developed, including large mixture of experts \cite{mixtureofexperts} or gating \cite{eigen_gating,cho_gating}. Our method can be seen as introducing both forms of routing: only accessing memories where mentions are detected is a form of gating and each of the entities accessed acts as an expert on its own subject. \tf{Clarify.}

\paragraph{OpenQA} We also test our model on Open-domain question answering, where a system must answer questions without a context document containing the gold answer. Most approaches to this problem focus on the \emph{open-book} setting, where a system first retrieves a set of documents from a large corpus and/or knowledge base then uses these documents to predict an answer through span prediction \cite{orqa, min_hardem, min_graphretriever, realm}. To test the ability of our model to encode world knowledge, we focus on the more challenging \emph{closed-book} setting, where no external knowledge or context is retrieved. Instead, the model must parse a query and rely on any potential knowledge encoded in its parameters to answer the question. \citet{relic} showed that a dual-encoder model of sentence and entity representations was able to predict the right entity for many of the questions in the TriviaQA dataset \cite{triviaqa} without access to any context document. This approach is most similar to ours, since we also frame the question answering problem as an entity prediction one. However, in contrast with \citet{relic}, we use the entity representations in the memory layer inside our model to inform the predictions and shows that this memory access improves the results. More recently, \citet{t5_openqa} fine-tuned the large transformer language models of \citet{t5} to generate answers to questions without access to the context. They show that their biggest model (comprising 11 billion parameters) is competitive with open-book approaches on three open question answering datasets. Though it is hard to compare the two approaches since the frame the prediction differently, our model achieves comparable performance to \citet{t5_openqa} despite only using 3\% of the parameters.



